Unconfused Ultraconservative Multiclass Algorithms

We tackle the problem of learning linear classifiers from noisy datasets in a multiclass setting. The two-class version of this problem was studied a few years ago by, e.g. Bylander (1994) and Blum et al. (1996): in these contributions, the proposed approaches to fight the noise revolve around a Perceptron learning scheme fed with peculiar examples computed through a weighted average of points from the noisy training set. We propose to build upon these approaches and we introduce a new algorithm called UMA (for Unconfused Multiclass additive Algorithm) which may be seen as a generalization to the multiclass setting of the previous approaches. In order to characterize the noise we use the confusion matrix as a multiclass extension of the classification noise studied in the aforementioned literature. Theoretically well-founded, UMA furthermore displays very good empirical noise robustness, as evidenced by numerical simulations conducted on both synthetic and real data. Keywords: Multiclass classification, Perceptron, Noisy labels, Confusion Matrix

==> Blum_up.tex <==
%here is the convergence proof%

\subsection{Convergence result} \label{sec:Analysis:Conv}

\iffalse
We will take a closer look at the margin properties of
$\xup{pq}$. We will also describe a way to choose $p$ and
$q$ based on the performance of the current classifier $W$.

We start by defining the set ``\emph{induced}'' by $\xup{pq}$ 
which is the set
all the $x_i$ used to compute $\xup{pq}$ from 
\eqref{eq:UpnAl:defGamma} :

\begin{align} \label{eq:Set:defExup}
  x_i \in \bigG(\xup{pq}) \iff t_i = q \wedge x_i \in \setA{p}
\end{align}

From \eqref{eq:Set:defExup} we define the \emph{size} of
$\xup{pq}$ as 

\begin{align} \label{eq:Set:defSize:1}
  \size{\xup{pq}} = \vert \bigG(\xup{pq}) \vert
\end{align}

\eqref{eq:Set:defSize:1} can be rewritten as

\begin{align} \label{eq:Set:defSize:2}
  \size{\xup{p,q}} = \sum_
  {\substack{\V{x}_i \in \setA{p} \\ t_i = q}} 1
\end{align}

And eventually \eqref{eq:Set:defSize:2} can be computed
indirectly in a similar way than $\gammapt{q}{p}$ 
following \eqref{eq:UpnAl:InvmatrixSystem}
\footnote{As long as Assumption \ref{As:UpnAl:UKDistri} hold,
note that $\size{\xup{pq}} = \infty$}
.

\bigskip

\fi

This section deal with the inherent approximation due to the
impossibility to directly compute expectation over $\UKDistri$.

One common solution (\cite{blum96polynomialtime}, 
\cite{bylander94learning}) is to assume that $z_{pq}$ is close  
to its expectation.

\begin{proposition}[closeness to expectation]
  As long as 
  $$ \vert \lbrace \V{x}_i | \V{x}_i \in \setA{p} \wedge t_i
  = q \rbrace \vert > N_0$$
  
  with high probability, the following holds :
  $$ 	\norm{\xup{pq} - \Ex{\V{X} \sim \UKDistri}{\xup{pq}}}
	< \epsilon . \V{1} $$
	
	And incidentally :
	\begin{equation}
	  \setA{p} =  \lbrace \V{x}_i | \forall k,
      \dotProd{\V{w}_k}{\V{x}_i} 
      - \dotProd{\V{w}_p}{\V{x}_i} 
      < - \sqrt{d} \epsilon \rbrace
      \end{equation}
      
      \begin{equation}
      \E{\margin} = \margin - \sqrt{d} . \epsilon
      \end{equation}
	
  \label{prop:closeness}
\end{proposition}
\begin{proof}
Stuff
\end{proof}

\iffalse

We now have to drop Assumption \ref{As:UpnAl:UKDistri}, and consider 
that expectation over $\UKDistri$ are actually not computable. 
However, given a large 
enough training set, we can assume that $\xup{pq}$ is fairly
close to its expectation, hence, our result stay mostly true,
with respect to the quantities manipulated.
This is a common assumption, (\emph{Blum}, \emph{Bylander})
and can be states as follows :

As long as $\size{\xup{p,q}} > N_0$

%\begin{align} \label{eq:Set:xupConv}
%  - \epsilon . \V{1} 
%  < \xup{p,q} - \Ex{}{\xup{pq}}
%  < \epsilon . \V{1}
%\end{align}

\begin{align} \label{eq:Set:xupConv}
	\norm{\xup{pq} - \Ex{\V{X} \sim \UKDistri}{\xup{pq}}}
	< \epsilon . \V{1}
\end{align}

where this inequality has to be taken element wise, with $\vert . \vert$ the
usual absolute value.

This is also tied to the definition of $\setA{p}$ in
\eqref{eq:UpnAl:defA} and we can now give a 
more precise form to $\setA{p}$

\begin{align} \label{eq:BUp:newA}
  \setA{p} =  \lbrace \V{x}_i | \forall k,
      \dotProd{\V{w}_k}{\V{x}_i} 
      - \dotProd{\V{w}_p}{\V{x}_i} 
      < - \sqrt{d} \epsilon \rbrace
\end{align}

Also it is worth noting that \eqref{eq:UpnAl:defA}
implies that 

\begin{align} \label{eq:Set:XupCrit}
  \forall \V{x} \in \bigG(\xup{pq}) : \margin_{pq}(\V{x}) < 
  - \norm{\epsilon . \V{1}} = - \sqrt{d} \epsilon
\end{align} 

 A concern that arises with the removal of
Assumption \ref{As:UpnAl:UKDistri}
is the confidence of $\xup{pq}$. 
As the algorithm make less and less mistakes,
the number of point used to compute $\xup{pq}$ is smaller. 
Here $N_0$ is some kind of threshold. 
Past it, we consider $\xup{pq}$ unreliable for making update.
This is actually not a problem as this very situation implies that 
we already have a good classifier (from \eqref{eq:UpnAl:defGamma}). 

\begin{align}
 \size{\xup{pq}} < N_0 \Leftrightarrow
     \vert \lbrace \V{x}_i | y_i = p \wedge t_i = q \rbrace
     \vert
     < N_0
\end{align}

Which means that there are only a few points of true class
$q$ for which $\dotProd{w_{pq}}{x_i} < 0$.

Remark that, as $w_{pq}$ is modified by any update implicating 
the class $p$ or $q$. For a given $p,q$, $\xup{pq}$ 
can be for a time lower than $N_0$ and then become greater later on. 

\bigskip

\Ugo{I dropped conditionning for $\Ex{}{\V{z}_{pq}}$ to lighten
a bit the notation} \\
Following \emph{Blum} we have two main results  :

\begin{align}
	\dotProd{\V{w}^*_{pq}}{\xup{pq}} & = 
           \dotProd{\V{w}^*_{pq}}
            {\xup{p,q} + \Ex{}{\xup{pq}} - \Ex{}{\xup{p,q}}} \\
	& = \dotProd{\V{w}^*_{pq}}{\xup{pq} - \Ex{}{\xup{pq}}} 
            + \dotProd{\V{w}^*_{pq}}{\Ex{}{\xup{pq}}} \\
        & \geq \dotProd{\V{w}^*_{pq}}{\Ex{}{\xup{pq}}} 
            - \norm{\epsilon . \V{1}} \\
	& \geq \margin_{pq} - \sqrt{d}\epsilon \label{eq:Blum:marginW*}
\end{align}

and

\begin{align}
	\dotProd{\V{w}_{pq}}{\xup{p,q}}  & = 
            \dotProd{\V{w}_{pq}}
            {\xup{p,q} - \Ex{}{\xup{p,q}} + \Ex{}{\xup{p,q}}} \\
        & = \dotProd{\V{w}_{pq}}{\xup{p,q} - \Ex{}{\xup{p,q}}}
            + \dotProd{\V{w}_{pq}}{\Ex{}{\xup{p,q}}} \\
        & \leq \dotProd{\V{w}_{pq}}{\Ex{}{\xup{p,q}}}
            + \norm{\epsilon . \V{1}} \\
	& \leq -\sqrt{d}\epsilon + \sqrt{d}\epsilon \\
	& \leq 0
\end{align}

Since, from \ref{eq:Set:xupConv} we have that, for any vector 
$\V{v}$

\begin{align}
  & \norm{\xup{pq} - \Ex{}{\xup{pq}}}
  . \cos(\V{v}, \xup{pq} - \Ex{}{\xup{pq}})
   \geq - \norm{\xup{pq} - \Ex{}{\xup{pq}}}
  > - \norm{\epsilon . \V{1}}  \\
  & \norm{\xup{pq} - \Ex{}{\xup{pq}}}
  . \cos(\V{v}, \xup{pq} - \Ex{}{\xup{pq}})
   \leq \norm{\xup{pq} - \Ex{}{\xup{pq}}}
  <  \norm{\epsilon . \V{1}} 
\end{align}

and

\begin{align}
  \norm{\V{w}_{pq}} = 1
\end{align}

Hence we have a sequence of update, all with margin at least : 
$\margin_{pq} - \sqrt{d}\epsilon  = \margin^{new}_{pq}$ 
and which are misclassified by the current classifier.

From \emph{Crammer and Singer}, as reminded
in Theorem \ref{Th:Set:MultiNovikoff}, we have that any additive 
multiclass algorithm will converge in
 $2 / {(\margin^{new}_{pq})}^2$ steps.
 
 \fi

\bigskip

\input{criterion}

\subsection{Selecting $p$ and $q$}

Although we can generate misclassified data, the question of 
selecting optimal $p$ and $q$ for $A_{pq}$ still remain. 
Intuitively we want the couple $(p,q)$ on which the current
classifier make the most errors. First because this update will
likely lead to a greater reduction of the error, then, and more
importantly, because $\xup{pq}$ will be more reliable.

However,an other wise strategy for selecting $p$ and $q$ 
might be to select the couple $(p,q)$ for which the
corresponding entry of the prediction confusion matrix
$\H{\Conf}_{pq}$ is maximal.

From these two strategies we propose two possible computation
for $(p,q)$

\begin{align}
  &(p,q)_{\terror} = \arg\max_{(p,q)} \size{\V{z}_{pq}} \\
  &(p,q)_{\tconf} = \arg\max_{(p,q)} p(\hat{y_i} = p | t_i = q)
    \approx \arg\max_{pq} \frac{\size{\xup{p,q}}}{p(t=q)}
\end{align}

However, the confusion strategy need a little more computation
as we have to estimate $p(t(x)=q)$.

We define $T = \left[ T_1 \cdots T_Q \right]^\intercal \in \realset^{Q}$ 
and $Y = \left[ Y_1 \cdots Y_Q \right]^\intercal \in \realset^Q$ as

\begin{align}
  T_p = p(\V{T} = p)
\end{align}

\begin{align}
  Y_q = p(\V{Y} = q)
\end{align}

\begin{align}
  Y_q = \sum_{p = 1}^Q p(\V{Y} = p | \V{T} = q) \times p(\V{T} = q)
\end{align}

And, in a same way than in \eqref{eq:UpnAl:InvmatrixSystem}, 
we can estimate $P$ as follow 

\begin{align}
  P = C^{-1} \times Y
\end{align}

==> analysis.tex <==
\section{Analysis} \label{sec:Analysis}

\begin{theorem} \label{Th:MultiNovikoff} Let $(x_1, t_i) \cdots
  (x_N, t_N)$ any sequence of labelled example.  Assume that there
  exists $W^*$ a perfect classifier with margin $\margin_0$. Then any
  multi-class additive algorithm does not make more than $2 /
  {\margin_o}^2$ update \footnote{An update is a step where $W$ is
    modified} .
\end{theorem}

\input{Blum_up}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "unconfused"
%%% End: 


==> criterion.tex <==
%Section about YAWP  and stopping criterion

\subsection{Stopping Criterion : two make one} \label{sec:Analysis:Crit}

While Theorem \ref{Th:MultiNovikoff} provide bound on the
number of update. We will actually never have to go that far.
Indeed we will systematically reach the situation where we
make less than $N_0$ error for each class, thus invalidating
Proposition \ref{prop:closeness}. Still, Theorem \ref{Th:MultiNovikoff}
is core to our result as it state that a solution exists. However
we will stop just before achieving it. Practically however,
we just have to track the error rate as stopping criterion.

\iffalse

We now take a closer look at the stopping criteria. One has
already been exhibited, and we will come back on it. We will
then introduce a new criterion derived from 
more practical consideration.
\bigskip

The criterion from  Theorem \ref{th:Set:MultiNovikoff}
is a purely
theoretical criterion which gives us a guarantee on the
maximal number of updates that have to be made to obtain 
a good classifier. In the case of the Unconfused perceptron
algorithm, note that each step lead to an update of $W$, then
this Theorem gives us a direct bound on the number of step
to perform.

One interesting fact is that the update vector does not need
to be true example. Thus, any sequence of point with the
same margin probability leads to the same bound. Thus
feeding the algorithm with average estimate, as we do,
does not modify this result. 

\bigskip

The other criterion has actually already been introduced
previously. We we have to keep in mind, when computing
update is that because of the drop of Assumption 
\ref{As:UpnAl:UKDistri}, we work on estimated quantities.
This means that we need to have enough data to actually
make estimation, therefore, we have to stop when
accurate estimation cannot be made.
More precisely, if 

\begin{align}
  \forall (p,q), \size{\xup{pq}} < N_0
\end{align}

then we can no longer make update. Eventually, this is 
not a problem as it implies that we already have a good 
classifier that make less than $N_0$ mistake.
One consequence of it is that we have a lower
bound on the empirical confusion risk attainable with our
algorithm since

\begin{align}
  \hat{C}_{pq} \geq \frac{N_0}{\sum_{\substack{\V{x}_i \in S \\ t_i = q}} 1} 
\end{align}

The relation between these two criteria is quite interesting.
While the first gives us guarantee that we will converge in a finite
number of step. The second one says that we will inevitably stop
before this number of step has been made. Practically we can only
consider the second result, but we need the first one to be sure
that we have a (unattainable) objective in a finite number of step.

\fi







==> discussion.tex <==
\section{Discussion}  \label{sec:Discuss}


\subsection{The non linear case}

The additional difficulty we want to tackle is when there is
no possible perfect linear classifier for our problem. This is 
an interesting case because, contrary to the \emph{true label} 
problem, it is hard to determine if a linear classifier
exists, given a noisy training set. Thus, our target
classifier will no longer be $W^*$ but $\E{W}$, and more
precisely its \emph{prediction confusion matrix} $\E{C}$.

Thus our goal now is to learn a classifier that is the closest possible
of $\E{W}$ in term of risk. However there is many possible comparison
between two classifiers, and some are more relevant than others.
For instance, we already argued on the fact that the error risk
seemed us less informative than the confusion risk.
If it is impossible to make no mistake,
then the closeness to the target classifier
can vary a lot with respect to the risk considered.

An other point to take care of is the non-uniqueness of the solution.
Actually, for a given target $\E{W}$ there is many
possible $W$ which achieve the same risk (error-wise or 
confusion-wise) but are drastically different from one to the other.
The worst case is the one which appears when we use the error risk
(i.e. minor classes are ignored in some cases). While directly 
minimizing the difference between confusion risk is an
effective work around for this problem, it still has flaw.
Indeed, in many multi-class problem, all classes are not equal. And
one can be easier to learn than other, thus mistakes on some are more
meaningful than mistakes on others. This is a level of detail
inaccessible if we simply look at the norm of the prediction
confusion matrix. And, once again, very different classifier can
be consider evenly good even if they are not from an higher level
point of view.

Eventually it all comes to granularity, and we have to choose which
level of granularity we consider in our problem (error on the dataset
as a whole, error rate within each class, class-wise error, $pq$-wise). 
This is not a problem that arise intuitively because in the perfect
case, all these granularity levels collapse.

\begin{align}
  \dist_{error}(\E{W}, W) = & \vert
      \risk_{error}(\E{W}) - \risk_{error}(W) \vert \\
  \dist_{confusion}(\E{W}, W) = & \vert
      \risk_{conf}(\E{W}) - \risk_{conf}(W) \vert \\
  \dist_{classwise}(\E{W}, W) =  & \Ex{}{\norm{\EV{c} - \hat{\V{c}}}} 
      \\
  \dist_{couplewise}(\E{W}, W) = &  \Ex{}{\fro{\E{C} - \hat{C}}}
\end{align}

With $c$ (resp $\EV{c}$) the reduced confusion vector

\begin{align}
  c_q = & \sum_{\substack{p = 1 \\ p \neq q}}^Q C_{pq} \\
  = & 1 - C_{qq}
\end{align}

Note that all of these distance (except the first one)
are compatible with \eqref{eq:Set:confRisk} as the risk.
Also, we assume that our target is one of the \emph{best} classifier
possible. Hence that $\hat{C} \geq \E{C}$ 
(resp ($\hat{\V{c}} \geq\EV{c}$) 
element-wise.
In the other case, we can only guarantee that the learned 
classifier will be
at least as good as the target one. Thus, the distance is not
(in this particularly case) the smallest possible.

Of course we could use even more precise error measure, we think
it would be overkill for the problem we want to tackle as our goal
is precisely to learn classes, and not something more complex.
Note however that the uniqueness of the solution is still not
guaranteed, but, with respect to our goal, we have reduced
potential solutions to equivalent ones in the couple-wise case.

\bigskip

To introduce the last stopping criterion smoothly, we have to see
an other interpretation of our problem.
We can actually consider that the computation of $\xup{}$ allow
us to somehow access to the true labeled example, in the sense
that we have access to example with their true class. We argued then
that these new points are likely to be real points as they result from 
an average of already observed example.

==> header.tex <==
% -*- coding: utf-8 -*-
\usepackage{amsmath,amsfonts}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{bm} %bold math

\usepackage{xspace}
\usepackage{graphicx}
\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{tikz}

\usepackage{algorithm}
\usepackage{algorithmic}

%\RequirePackage{algorithmic}
\RequirePackage{color}

% ajout Ugo

\newcommand\Ugo[1] {\textcolor{blue}{\textbf{UL : #1}}}
\newcommand\Todo[1] {\textcolor{green}{\textbf{TODO : #1}}}
\newcommand\V[1] {\bm{#1}} %vector
\newcommand\Ex[2] {\mathbb{E}_{#1} \left[ #2 \right]} %expectation (long version)
\newcommand\dotProd[2] {\left< {#1} , {#2} \right>}
\newcommand\norm[1] {\Vert {#1} \Vert}
\newcommand\UKDistri{\mathcal{D}}
\newcommand\setA[1]{\mathcal{A}_{#1}}
\newcommand\gammapt[2]{\gamma_{#1}^{\setA{#2}}}
\newcommand\gammalong[2]{\Ex{p(\V{x}_i | t_i = p)}{\V{x}_i}}
\newcommand\mupt[2]{\mu_{#1}^{#2}}
\newcommand\mulong[2]{\Ex{p(\V{x}_i | y_i = p)}{\V{x}_i}}
\newcommand\xup[1]{\V{z}_{#1}}
\newcommand\size[1]{\vert {#1} \vert_S}
\newcommand\fro[1]{\norm{{#1}}_F}
\newcommand\EV[1]{\E{\V{#1}}} %expectation of a vector
\newcommand\E[1]{\widetilde{#1}} %expectation
\renewcommand\H[1]{\widehat{#1}}
\newcommand{\confusion}{{\cal C}}
\newcommand{\classes}{{\cal Q}}

%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{example}{Example}

\renewcommand{\iff}{\Leftrightarrow}
%\newcommand\Up[1]{\overline{#1}} %'upperline'
%\newcommand\UV[1]{\Up{\V{#1}}} %vector 'upperline'
%\newcommand\Ident{\V{I}} %identity matrix
\newcommand{\uma}{{\tt UMA}\xspace}
\newcommand{\margin}{\theta}
\renewcommand{\algorithmicensure}{{\bf Output:}}
\renewcommand{\algorithmicrequire}{{\bf Input:}}


%%% Theorems, etc
%%%
%%% Comments
\newcommand{\liva}[1]{\textcolor{red}{{\bf (Liva:} #1{\bf )}}}

\newcommand{\ontop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
\newcommand{\indicator}[1]{\mathbb{I}{\left\{ #1 \right\} }}
\DeclareMathOperator*{\argmax}{\text{argmax}}
\DeclareMathOperator*{\argmin}{\text{argmin}}

%%% Misc. shortcuts
\def\algo{\mathcal{A}}
\def\inputset{\mathcal{S}}
\def\trainingset{\mathcal{S}}
\def\inputz{\mathcal{Z}}
\def\distribution{D}
\def\proba{\mathbb{P}}
\def\inputspace{\mathcal{X}}
\def\outputspace{\mathcal{Y}}
\def\targetspace{\mathcal{Y}}
\def\productspace{\mathcal{Z}}
\def\proba{\mathbb{P}}
\def\expectation{\mathbb{E}}
\def\realset{\mathbb{R}}
\def\naturalset{\mathbb{N}}
\def\integerset{\mathbb{Z}}
\DeclareMathOperator*{\union}{\cup}
%\newcommand\union{\cup}
\def\inter{\cap}
\def\family{\mathcal{H}}
\def\loss{\ell}
\def\risk{R}
\def\distributions{\mathcal{D}}
\def\rank{\text{rank}}
\def\pac{\xspace{\sc Pac}}
\def\pefc{\text{\sc Pefc}}
\def\auc{\text{\sc Auc}\xspace}
\def\roc{\text{\sc Roc}\xspace}
\def\sign{\text{sign}}
\def\np{\text{\sc Np}}
\def\normal{\mathcal{N}}
\def\identity{I}
\def\iid{{\sc IID}\xspace}
\def\hypothesis{H}
\def\hypotheses{\mathcal{H}}
\def\variance{\mathbb{V}}
\def\test{\text{test}}
%%% Bold font
\def\bfell{\boldsymbol{\ell}}
\def\bfzero{\boldsymbol{0}}
\def\bfx{\boldsymbol{x}}
\def\bfa{\boldsymbol{a}}
\def\bfz{\boldsymbol{z}}
\def\bfh{\boldsymbol{h}}
\def\bfZ{\boldsymbol{Z}}
\def\bfz{\boldsymbol{z}}
\def\bfD{\boldsymbol{D}}
\def\bfC{\boldsymbol{C}}
\def\bfP{\boldsymbol{P}}
\def\bfQ{\boldsymbol{Q}}
\def\bfS{\boldsymbol{S}}
\def\bfs{\boldsymbol{s}}
\def\bfX{\boldsymbol{X}}
\def\bfY{\boldsymbol{Y}}
\def\bfu{\boldsymbol{u}}
\def\bfv{\boldsymbol{v}}
\def\bfw{\boldsymbol{w}}
\def\bfy{\boldsymbol{y}}
\def\bfpi{\boldsymbol{\pi}}
\def\bfalpha{\boldsymbol{\alpha}}
\def\bfmu{\boldsymbol{\mu}}
%Ugo
\def\UCPA{\text{UCPA}}
\def\UCPAlong{\textit{UnConfused Passive Aggressive}}
\def\UMA{\text{UMA~}}
\def\PA{\text{PA}}
\def\PAlong{\textit{Passive Aggressive}}
\def\Pdim{\text{Pdim}}
%\def\margin{m}
\def\Conf{C}
\def\dist{\text{dist}}
\def\terror{\text{error}}
\def\tconf{\text{conf}}
\def\tcorrect{\text{corr}}
\def\tmixt{\text{mixt}}
\def\tother{\text{other}}
\def\bigE{\mathcal{E}}
\def\bigG{\mathcal{G}}
\def\bigC{\mathcal{C}}
\def\bigO{\mathcal{O}}
\def\bigH{\mathcal{H}}
\def\bigF{\mathcal{F}}
\def\bigI{\mathcal{I}}
\def\bigJ{\mathcal{J}}
\def\bigN{\mathcal{N}}
\def\bigM{\mathcal{M}}
\def\diag{\text{diag}}
\def\err{\text{err}}

%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SMALL EQUATIONS

\usepackage{exscale}
\makeatletter
\newenvironment{equationsize}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \equation
}{\endequation \ignorespacesafterend} 
\makeatother

\makeatletter
\newenvironment{equationsize*}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \equation
}{\nonumber\endequation \ignorespacesafterend} 
\makeatother


\makeatletter
\newenvironment{alignsize}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \align
}{\endalign \ignorespacesafterend} 
\makeatother

\makeatletter
\newenvironment{alignsize*}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \start@align\@ne\st@rredtrue\m@ne
}{\endalign\ignorespacesafterend} 
\makeatother

%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 

